Detect \& Score: Privacy-Preserving Misbehaviour Detection and Contribution Evaluation in Federated Learning

Federated learning with secure aggregation enables private and collaborative learning from decentralised data without leaking sensitive client information. However, secure aggregation also complicates the detection of malicious client behaviour and the evaluation of individual client contributions to the learning. To address these challenges, QI (Pejo et al.) and FedGT (Xhemrishi et al.) were proposed for contribution evaluation (CE) and misbehaviour detection (MD), respectively. QI, however, lacks adequate MD accuracy due to its reliance on the random selection of clients in each training round, while FedGT lacks the CE ability. In this work, we combine the strengths of QI and FedGT to achieve both robust MD and accurate CE. Our experiments demonstrate superior performance compared to using either method independently.

==> CIFAR10_hetero_m_5.tex <==
2.000000000000000000e+00,3.007692307692307887e-01,4.001381075065285065e-01,5.161666979391437149e-01,9.813438431052681765e-02,5.034040772279347875e-01,3.414376275897921253e-01,4.588385874232648876e-01,4.432403959172974695e-01,5.890929999609899603e-01
3.000000000000000000e+00,3.516669441669441620e-01,3.427782503014701332e-01,4.120796308954203790e-01,7.489573648270098083e-02,6.284381518511873432e-01,2.013481757870533018e-01,4.842083248158869369e-01,2.576429182902663095e-01,5.665163435005744486e-01
4.000000000000000000e+00,4.606837606837607124e-01,3.620963831490147666e-01,4.831343063541206351e-01,1.738612176919832053e-01,7.475063036755382750e-01,2.109271809721348090e-01,5.132655853258947243e-01,3.645258184814956781e-01,6.017427942267455920e-01
5.000000000000000000e+00,5.593663199545553244e-01,3.577325890483785131e-01,5.691520467836256314e-01,3.317356993931818154e-01,7.869969405159288334e-01,1.847716771099802979e-01,5.306935009867767006e-01,4.022956220287050577e-01,7.360084715385462051e-01
6.000000000000000000e+00,5.401856476856476963e-01,3.616300366300366220e-01,6.041809497691850162e-01,2.934178814538776492e-01,7.869534139174176879e-01,1.553785782340091071e-01,5.678814950260641092e-01,3.759556250969278146e-01,8.324062744414422177e-01
7.000000000000000000e+00,5.734536215418568617e-01,4.095579858737753431e-01,5.533151059466848709e-01,3.516407028436223658e-01,7.952665402400913575e-01,2.270497459062613133e-01,5.920662258412894285e-01,3.221644325891914740e-01,7.844657793041782679e-01
8.000000000000000000e+00,5.747523228405582163e-01,4.421367521367521869e-01,6.390044166359956090e-01,3.520822795691532225e-01,7.974223661119632656e-01,3.069815193239582296e-01,5.772919849495461442e-01,3.917814307823962450e-01,8.862274024895949731e-01
9.000000000000000000e+00,5.465471946354300004e-01,4.953187447227694884e-01,6.892477405635301091e-01,3.132027422840787945e-01,7.798916469867811507e-01,3.541998039731572567e-01,6.364376854723816646e-01,4.262497434934651719e-01,9.522457376335951018e-01
1.000000000000000000e+01,6.189678295560648857e-01,3.896553884711779214e-01,5.859848484848485528e-01,4.896647887594888227e-01,7.482708703526409488e-01,2.264879308160731297e-01,5.528228461262827409e-01,3.162088875467178317e-01,8.557608094229792739e-01
1.100000000000000000e+01,6.425789406671759130e-01,5.867890881048775098e-01,7.429079254079253847e-01,5.353918026508517336e-01,7.497660786835000923e-01,4.761103345674071452e-01,6.974678416423478744e-01,5.103495662380220788e-01,9.754662845778286906e-01
1.200000000000000000e+01,5.601748251748251972e-01,5.115384615384614975e-01,7.171304134462028745e-01,3.271689596611834228e-01,7.931806906884669717e-01,2.860839336920519838e-01,7.369929893848710112e-01,4.939789347971156874e-01,9.402818920952900061e-01
1.300000000000000000e+01,5.643414918414918491e-01,4.924667437825333005e-01,7.362757125915020406e-01,3.298458774817109029e-01,7.988371062012727952e-01,2.818412295115967359e-01,7.030922580534698652e-01,4.969730970940291481e-01,9.755783280889749332e-01
1.400000000000000000e+01,5.643414918414918491e-01,5.074633699633699369e-01,7.713184476342369589e-01,3.298458774817109029e-01,7.988371062012727952e-01,2.899689560732788829e-01,7.249577838534609908e-01,5.161622807718500017e-01,1.026474614496623916e+00
1.500000000000000000e+01,5.643414918414918491e-01,4.520146520146520186e-01,7.383569646727541347e-01,3.298458774817109029e-01,7.988371062012727952e-01,2.707074410702535738e-01,6.333218629590504634e-01,4.949526638887475904e-01,9.817612654567606789e-01
1.600000000000000000e+01,5.643414918414918491e-01,4.572795178677531713e-01,7.523429786587680912e-01,3.298458774817109029e-01,7.988371062012727952e-01,2.160588453209762172e-01,6.985001904145301532e-01,5.036067049675276852e-01,1.001079252350008497e+00
1.700000000000000000e+01,5.716142191142192797e-01,5.277610246650493719e-01,7.920255183413077438e-01,3.311269323591349290e-01,8.121015058693036304e-01,3.008798994873441712e-01,7.546421498427545727e-01,5.264082827543521415e-01,1.057642753928263346e+00
1.800000000000000000e+01,5.815043290043291346e-01,5.493771862812110163e-01,7.689485952643847488e-01,3.374136663159256755e-01,8.255949916927325383e-01,3.194065741795393265e-01,7.793477983828827060e-01,5.125376106737491444e-01,1.025359579855020353e+00
1.900000000000000000e+01,5.600757575757576712e-01,5.142689611729859278e-01,7.991683754841648613e-01,3.191976268226426328e-01,8.009538883288727096e-01,3.385652440251832318e-01,6.899726783207886793e-01,5.751745368892215993e-01,1.023162214079108123e+00
2.000000000000000000e+01,5.715043290043290147e-01,4.999832468872716373e-01,8.356152619310514007e-01,3.263302312865021260e-01,8.166784267221558480e-01,3.112756779237171312e-01,6.886908158508261435e-01,6.172931189986430311e-01,1.053937404863459770e+00


==> CIFAR10_homo_m_5.tex <==
2.000000000000000000e+00,9.611111111111110272e-01,5.409399810715600498e-01,5.121025603223745559e-01,8.999999999999999112e-01,1.022222222222222143e+00,3.898940628201660319e-01,6.919858993229540678e-01,3.799034182407075577e-01,6.443017024040416096e-01
3.000000000000000000e+00,1.000000000000000000e+00,5.687931951089846283e-01,6.365513141828931243e-01,1.000000000000000000e+00,1.000000000000000000e+00,4.095715169586985338e-01,7.280148732592707228e-01,5.069470556184555443e-01,7.661555727473307043e-01
4.000000000000000000e+00,1.000000000000000000e+00,6.721356421356421418e-01,7.872766122766122754e-01,1.000000000000000000e+00,1.000000000000000000e+00,5.022769217006022302e-01,8.419943625706820534e-01,6.630800952237581036e-01,9.114731293294664471e-01
5.000000000000000000e+00,1.000000000000000000e+00,6.926563632445985608e-01,7.830659536541890731e-01,1.000000000000000000e+00,1.000000000000000000e+00,5.053442629044905265e-01,8.799684635847065950e-01,5.803556838392789352e-01,9.857762234690992109e-01
6.000000000000000000e+00,1.000000000000000000e+00,6.946167557932263481e-01,8.536868686868686051e-01,1.000000000000000000e+00,1.000000000000000000e+00,5.954619710222321949e-01,7.937715405642205013e-01,7.535522663872831206e-01,9.538214709864540897e-01
7.000000000000000000e+00,1.000000000000000000e+00,6.507357408673197785e-01,9.038461538461538547e-01,1.000000000000000000e+00,1.000000000000000000e+00,5.176067047608396976e-01,7.838647769737998594e-01,8.150384575283883271e-01,9.926538501639193823e-01
8.000000000000000000e+00,1.000000000000000000e+00,7.681799194957088517e-01,9.347008547008546220e-01,1.000000000000000000e+00,1.000000000000000000e+00,5.829169599876083963e-01,9.534428790038093071e-01,8.479218179889130846e-01,1.021479891412796048e+00
9.000000000000000000e+00,1.000000000000000000e+00,8.218956482114376794e-01,9.365190365190365629e-01,1.000000000000000000e+00,1.000000000000000000e+00,6.651896468253968298e-01,9.786016495974785290e-01,8.629144209914527686e-01,1.010123652046620357e+00
1.000000000000000000e+01,1.000000000000000000e+00,9.173737373737372858e-01,9.241452991452991927e-01,1.000000000000000000e+00,1.000000000000000000e+00,8.424343168849887098e-01,9.923131578624858617e-01,8.249795095591800909e-01,1.023311088731418295e+00
1.100000000000000000e+01,1.000000000000000000e+00,8.918181818181818432e-01,9.464646464646463420e-01,1.000000000000000000e+00,1.000000000000000000e+00,8.125533087015683886e-01,9.710830549347952978e-01,8.775405167303756970e-01,1.015388776198916876e+00
1.200000000000000000e+01,1.000000000000000000e+00,9.340404040404038932e-01,9.380341880341880323e-01,1.000000000000000000e+00,1.000000000000000000e+00,8.611393070538518879e-01,1.006941501026956010e+00,8.559817930987152490e-01,1.020086582969660816e+00
1.300000000000000000e+01,1.000000000000000000e+00,8.383083583083582591e-01,9.298701298701299578e-01,1.000000000000000000e+00,1.000000000000000000e+00,7.054444136446947899e-01,9.711723029720217282e-01,8.036620196025315854e-01,1.056078240137728219e+00
1.400000000000000000e+01,1.000000000000000000e+00,8.591125541125540499e-01,9.222222222222221655e-01,1.000000000000000000e+00,1.000000000000000000e+00,7.372452597640200000e-01,9.809798484610880998e-01,7.231503014759008696e-01,1.121294142968543461e+00
1.500000000000000000e+01,1.000000000000000000e+00,8.985569985569984430e-01,9.512265512265513090e-01,1.000000000000000000e+00,1.000000000000000000e+00,7.808642403964097811e-01,1.016249756717586994e+00,8.626521182162716350e-01,1.039800984236830983e+00
1.600000000000000000e+01,1.000000000000000000e+00,8.769952269952270285e-01,9.909090909090909616e-01,1.000000000000000000e+00,1.000000000000000000e+00,7.526472367178107525e-01,1.001343217272643304e+00,9.636363636363637353e-01,1.018181818181818299e+00
1.700000000000000000e+01,1.000000000000000000e+00,8.845709845709844865e-01,9.742424242424242431e-01,1.000000000000000000e+00,1.000000000000000000e+00,7.608074690735237011e-01,1.008334500068445383e+00,9.200135449449294844e-01,1.028471303539919113e+00
1.800000000000000000e+01,1.000000000000000000e+00,8.758297258297258470e-01,9.742424242424242431e-01,1.000000000000000000e+00,1.000000000000000000e+00,7.550903148321205238e-01,9.965691368273311701e-01,9.200135449449294844e-01,1.028471303539919113e+00
1.900000000000000000e+01,1.000000000000000000e+00,9.457070707070707183e-01,9.818181818181818121e-01,1.000000000000000000e+00,1.000000000000000000e+00,8.670321808627816651e-01,1.024381960551359771e+00,9.454545454545454364e-01,1.018181818181818077e+00
2.000000000000000000e+01,1.000000000000000000e+00,9.595959595959595578e-01,9.818181818181818121e-01,1.000000000000000000e+00,1.000000000000000000e+00,9.097006503627131924e-01,1.009491268829205923e+00,9.454545454545454364e-01,1.018181818181818077e+00


==> ISIC_homo_m_5.tex <==
2.000000000000000000e+00,6.231546231546231107e-01,4.253846153846153610e-01,4.898304473304472273e-01,5.270774480999416145e-01,7.192317982093046069e-01,3.026334275129777263e-01,5.481358032562529958e-01,2.647834225612984982e-01,7.148774720995959564e-01
3.000000000000000000e+00,6.470760233918128046e-01,4.622589450453227222e-01,4.848260356774288238e-01,5.213053041172825974e-01,7.728467426663430118e-01,3.359077929848697242e-01,5.886100971057757203e-01,3.468522806478763765e-01,6.227997907069813266e-01
4.000000000000000000e+00,6.909829059829059039e-01,4.782679738562091165e-01,7.018721045036834250e-01,5.622349880520158827e-01,8.197308239137959252e-01,3.300248666339570813e-01,6.265110810784610962e-01,5.419154251978454129e-01,8.618287838095214370e-01
5.000000000000000000e+00,6.909829059829059039e-01,4.480428343586238538e-01,7.756835269993163084e-01,5.622349880520158827e-01,8.197308239137959252e-01,3.079885570875643408e-01,5.880971116296833667e-01,6.417658035237989722e-01,9.096012504748336447e-01
6.000000000000000000e+00,7.183333333333332682e-01,4.173659673659673719e-01,8.018939393939394922e-01,5.798661959030095847e-01,8.568004707636569517e-01,2.248960327437336537e-01,6.098359019882011456e-01,6.107000931190598170e-01,9.930877856688191674e-01
7.000000000000000000e+00,7.233333333333333837e-01,4.855375618533512849e-01,7.951515151515151647e-01,5.829238791829278732e-01,8.637427874837388941e-01,2.737364176079974953e-01,6.973387060987050745e-01,5.915151515151515493e-01,9.987878787878787801e-01
8.000000000000000000e+00,7.233333333333333837e-01,5.369396238436486835e-01,8.486868686868687117e-01,5.829238791829278732e-01,8.637427874837388941e-01,4.187471987734942003e-01,6.551320489138031666e-01,7.448176852657748537e-01,9.525560521079625698e-01
9.000000000000000000e+00,8.031313131313131404e-01,4.613539676697571146e-01,8.534487734487734567e-01,6.659370973955769379e-01,9.403255288670493428e-01,3.215035450534166062e-01,6.012043902860976230e-01,7.572231886820797175e-01,9.496743582154671959e-01
1.000000000000000000e+01,8.384848484848486105e-01,5.194307885097357858e-01,8.563852813852813606e-01,7.263877994914824665e-01,9.505818974782147546e-01,4.454218716089495822e-01,5.934397054105219338e-01,7.162659728236229206e-01,9.965045899469398005e-01
1.100000000000000000e+01,8.493939393939395899e-01,5.798819163292846524e-01,9.040404040404041996e-01,7.362694356306134225e-01,9.625184431572657573e-01,3.984098071810024955e-01,7.613540254775668092e-01,8.118773353995221154e-01,9.962034726812862839e-01
1.200000000000000000e+01,8.493939393939395899e-01,5.315360078517972209e-01,9.103535353535352481e-01,7.362694356306134225e-01,9.625184431572657573e-01,3.528366141662480637e-01,7.102354015373464335e-01,8.381538320054275903e-01,9.825532387016429059e-01
1.300000000000000000e+01,8.493939393939395899e-01,5.786623077644749147e-01,8.969336219336219163e-01,7.362694356306134225e-01,9.625184431572657573e-01,4.817102184188779002e-01,6.756143971100719847e-01,8.034506734144122309e-01,9.904165704528316017e-01
1.400000000000000000e+01,8.847474747474748380e-01,5.234619525641197590e-01,9.219336219336218274e-01,8.275674596449070775e-01,9.419274898500425985e-01,3.957267662905764594e-01,6.511971388376630587e-01,8.381638149196140031e-01,1.005703428947629652e+00
1.500000000000000000e+01,8.936363636363635621e-01,6.001044277360066959e-01,9.199134199134200163e-01,8.438966062490124154e-01,9.433761210237147088e-01,4.320204802665925659e-01,7.681883752054208259e-01,8.356163187660767822e-01,1.004210521060763250e+00
1.600000000000000000e+01,8.936363636363635621e-01,5.200918964076859385e-01,9.108225108225107558e-01,8.438966062490124154e-01,9.433761210237147088e-01,3.607200675933029399e-01,6.794637252220689927e-01,8.308620000887732004e-01,9.907830215562483112e-01
1.700000000000000000e+01,8.936363636363635621e-01,5.992188805346699843e-01,9.142968142968141976e-01,8.438966062490124154e-01,9.433761210237147088e-01,4.547833824238579070e-01,7.436543786454821170e-01,8.466834138925358744e-01,9.819102147010925208e-01
1.800000000000000000e+01,8.936363636363635621e-01,6.030284043441938024e-01,9.122766122766122754e-01,8.438966062490124154e-01,9.433761210237147088e-01,4.598842803366664511e-01,7.461725283517210983e-01,8.442373822656912274e-01,9.803158422875333233e-01
1.900000000000000000e+01,8.936363636363635621e-01,5.600865474394887134e-01,9.094988344988343965e-01,8.438966062490124154e-01,9.433761210237147088e-01,4.020840498095881177e-01,7.180890450693893090e-01,8.205318023205699918e-01,9.984658666770988011e-01
2.000000000000000000e+01,8.936363636363635621e-01,6.147506690076349756e-01,9.122766122766122754e-01,8.438966062490124154e-01,9.433761210237147088e-01,4.239497842972499431e-01,8.055515537180200081e-01,8.442373822656912274e-01,9.803158422875333233e-01

